LZR: Identifying Unexpected Internet Services

Internet-wide scanning is a commonly used research technique that has helped uncover real-world attacks, find cryptographic weaknesses, and understand both operator and miscreant behavior. Studies that employ scanning have largely assumed that services are hosted on their IANA-assigned ports, overlooking the study of services on unusual ports. In this work, we investigate where Internet services are deployed in practice and evaluate the security posture of services on unexpected ports. We show protocol deployment is more diffuse than previously believed and that protocols run on many additional ports beyond their primary IANA-assigned port. For example, only 3% of HTTP and 6% of TLS services run on ports 80 and 443, respectively. Services on non-standard ports are more likely to be insecure, which results in studies dramatically underestimating the security posture of Internet hosts. Building on our observations, we introduce LZR ("Laser"), a system that identifies 99% of identifiable unexpected services in five handshakes and dramatically reduces the time needed to perform application-layer scans on ports with few responsive expected services (e.g., 5500% speedup on 27017/MongoDB). We conclude with recommendations for future studies.

==> background.tex <==
\section{Background}

ZMap scans for TCP Handshakes --- sending a \syn Packet and collecting \sa responses --- is commonly used to detect whether an IP/Port is able to establish a TCP Connection (cite), and is used as a proxy to determine whether an IP/port is running the expected/assigned service on the port.

For example, the original zmap paper looked at \sa across all ports but did not investigate whether the \sa s being received are actually representative of established TCP connections.

Scanning for Liveness defines and analyzes ``liveness`` as any IP that either RSTs or Acknowledges a Syn Scan. Our work shows that such a definition is a misleading proxy for whether  TCP connection can actually be established with an IP, let alone whether the IP is running the expected application (e.g. HTTP on port 8080). 

NMap uses a \sa on a port as a proxy for that port running the expected service. 

\begin{enumerate}
    \item work assumes L4 is accurate proxy
    \item work had discrepancy b/w \# of s/as b/w L7 vs L4 but didnt investigate
\end{enumerate}


Some scanning work in the community commonly scans L7 using two steps: an L4 filtering step (ZMap) to figure out which IPs can complete a handshake and then an L7 filtering step (ZGrab) to verify that the IPs which \sa on a port actually run the scanned-for application layer. The implications of scanning twice in a row and how it effects the accuracy of scanning results has never been studied. 


In this work we find that as ports become less common, TCP handshakes are no longer accurate proxies for IP/Ports running services and can be up to three orders of magnitude off.

Though Inconsistencies between receiving a \sa and hosting a L7 service has been investigated before \textemdash Pearce et al., identifies \sa inconsistencies due to firewall behaviors and finds it affects less than 2\% of all scanned traffic on port 80 \cite{pearce2017augur} \textemdash the effects of \sa inconsistencies on security relevant , ephemeral, and other uncommon ports has not been formally quantified in details as we will do in the following sections. 


\rt{Moving this here as it is better in background.} Previous work often uses two phased scanning \cite{durumeric2013analysis,heninger2012mining}, in which two scans (one scanning Layer 4 and one scanning Layer 7) are paired back-to-back in order to fulfill symbiotic goals: the first scan is often used to discover hosts listening on a particular port and the second scan collects data about the service that is expected to be running on the particular port. A numerous amount of such previous work also provides evidence that the number of hosts which respond on the first scan (i.e., are listening on a particular port) is far greater than the number of hosts responding on the second scan (i.e., are hosting the expected service) \cite{mirian2016internet,springall2016ftp,holz2011ssl,amann2017mission,holz2015tls,checkoway2014practical}. However, the cause behind this mis-match in numbers has never been explained or empirically explored. 


==> majorRevision_Response.tex <==
\section{Addressed Major Revisions}

We thank the USENIX Security reviewers for their detailed comments and
suggestions. We sincerely believe your feedback and requested changes have
resulted in a significantly improved paper. We bold all requested changes and
detail the manner in which we addressed those requests below:

\begin{itemize}

    \item \textbf{Quantify the deployment of various defensive techniques by defense provided as a top-level result, and empirically evaluate the efficacy of these mechanisms:} We have included Section~\ref{sub:sec:efficacy} to evaluate the efficacy of the discovered middlebox protections.
    Concretely, we discuss the deployment of each defensive technique (i.e., what fraction of ASes each defensive technique appears in), how effective identifiable middleboxes are at preventing undesirable connections (e.g., DDoS), and quantitatively evaluate each defensive technique's ability to inadvertently slow down Internet-wide scanning and the spread of malware.
    We have also change the titles of Section~\ref{sub:sec:syn_sent} and Section~\ref{sub:sec:cont_sa} to emphasize the studied defensive technique, and the ordering and presentation of results throughout all subsections after Section~\ref{sub:sec:db1} in order to emphasize the deployment of the defensive techniques as the top-level result.

    \item \textbf{Add results for other ports in performance evaluation:}
    We have added an \textit{additional} seven port/protocol combinations in Table~\ref{table:comp_zgrabs} including popular assigned services, unpopular assigned services, and unassigned services (Table~\ref{table:comp_zgrabs} previously only included four assigned services).
    Furthermore, we add the expected performance of 99\% of all ports (i.e., unassigned ports) in the ``How much faster is is L7 scanning with \lmap'' paragraph of Section~\ref{sub:sec:lzr_eval}: ``Unpopular ports are expected to have the same performance improvement as 62220/HTTP (up to 25~times speed-up) because IPs on the majority of ports are more likely to not acknowledge data when sending a \sa''.

    \item \textbf{Categorize into "popular" v.s. "unpopular" services and present the results:} In Section~\ref{sub:sec:twophase}, we split ports between two "popular" and "unpopular" categories, which we define by using Grubbs's test for
    outliers~\cite{grubbs1950sample} with a 99.9\% confidence interval based on the
    total number \sa{s} and the presence of an expected service. We then changed all results that were previously presented as ranges to be the presented as an average across popular and unpopular ports.

    \item \textbf{Provide high-level overviews and highlight the key takeaway:}
    We added high-level overviews in the beginning of Section~\ref{sec:l4}, Section~\ref{sec:l7} and Section~\ref{sec:optimizations} and summaries that highlighted the key takeaways at the end of Section~\ref{sec:l4}, Section~\ref{sec:l7} and Section~\ref{sec:optimizations} (reviews were content with Section~\ref{sub:l4_heuristic}).

    \item \textbf{Carry out the work proposed in P2 in the rebuttal to "make this paper more applicable to the broader security community":}
    We have re-framed the paper to focus on the prevalence of unexpected services, how to find them, and why the security community must study them (the previous framing focused more on evaluating the accuracy of a scanning methodology, which is widely used in the security community).

    We have added Section~\ref{sub:sec:eval_security}, which
    compares the security of unexpected and expected services and shows that unexpected services are often even greater contributors to the Internet's vulnerability than expected services. Concretely, we evaluate the security of unexpected services in four different security contexts: widespread IoT devices, vulnerable TLS, prevalence of login pages, and SSH hygiene. Furthermore, we discuss how unexpected services
    affect the results of previous security studies (e.g., there are over twice as many certificates with a known private key than reported in previous work by Heninger et~al.\ and Hastings et~al.~\cite{heninger2012mining,hastings2016weak}).

    In Section~\ref{sub:sec:unexpected services}, we have added a new experiment and show how only a small fraction of IANA-assigned services are on their assigned port (e.g., only 5.5\% of Telnet resides on TCP/23) and the direct implications to future security studies (e.g., the number of infected devices due to botnets is potentially over 15~times worse than previously shown). We also provide examples of how organizations use unexpected ports to hide services (e.g., BBIN International in Section~\ref{sub:sec:unexpected services}).

    We give scanning recommendations to the security community in Section~\ref{sub:sec:unexpected services} and Section~\ref{sec:rec_conclusion}, including how to efficiently find targeted protocols (i.e., depending on the type of security question being asked) across unexpected ports in order to be able to conduct more comprehensive and accurate security studies.

    Furthermore, as stated earlier in this letter, we have included Section~\ref{sub:sec:efficacy}, which quantifies the deployment and efficacy of various middlebox defenses.

    \item \textbf{Report the overhead/improvement/cost in terms of packets and time, and compare LZR + ZGrab with LZR filtered addresses to ZGrab without LZR filtered addresses in packets and time:}
    In Section~\ref{sub:sec:lzr_eval}, we have added a completely new ``Bandwidth Savings'' experiment which evaluates LZR in terms of packets sent, and have added the evaluation of ZMap/LZR, ZMap/LZR + ZGrab, and Offline ZMap + LZR to Table~\ref{table:comp_zgrabs} for both ``Speed Up'' and ``Bandwidth Savings'' experiments. In all but one case, using LZR decreases scanning time, even if the amount of bandwidth used is higher than just ZGrab.

    \item \textbf{Acknowledge limitations more clearly, in particular that a new connection may be required if the LZR probe results in an unrecoverable error for a connection, thus it can result in overall higher cost for ports that are responsive in the majority of cases:}
    We have changed \lmap to send the expected handshake by default---as opposed to the previous design that sent two newlines---thereby reducing the chances of unrecoverable errors. Furthermore, we have included a completely new experiment and discussion (Section~\ref{sub:sec:consequences_handshake_order}) which investigates how sending unexpected data does not impact fingerprinting, but can cause up to 30\% of follow-up handshakes to temporarily fail.
    Furthermore, we discuss and showed potential bandwidth overhead in the ``How much bandwidth..?'' paragraph of Section~\ref{sub:l4_heuristic} and present accompanying data in Table~\ref{table:comp_zgrabs}.

    \item\textbf{Fix the small text issues in Figures~\ref{fig:l4_all},~\ref{fig:l4_no_establish}, and \ref{fig:hist_services}:} We have widened and enlarged Figures~\ref{fig:l4_all},~\ref{fig:l4_no_establish}, and \ref{fig:hist_services}.

\end{itemize}


==> methodology.tex <==
\section{Methodology}


\subsection{Differentiating Categories of IP Responses across L4}

When scanning the internet, our true intention is to measure \textit{hosts} and not \textit{IPs}, where we define an IP as an IP address and a host as the actual server behind the IP address. We fingerprint servers by looking for identifiers within the L7 layer (e.g., host keys on port 22, certificate fingerprint on port 443, etc). However, IP addresses are currently the only way to reach a host, therefore making it necessary to study how closely correlated are IPs and hosts.


When scanning, we prioritize hosts which run applications (HTTP, SSH) that we can engage with. Note that the application need not be public (we do not expect to be able to SSH into every SSH service), but we expect the application to speak the appropriate protocol to inform us of a service not meant for our scanner. 

...

We also find the need to differentiate a service, an established connection, and just a S/A, because we find that all S/Aing IPs cannot necessarily establish a connection, let alone host a service. 

\todo{These are all categories of what? IP ``Behavior``? whats another word for behavior?}

\begin{itemize}
    \item Service: (IP, Port, L4, L7)
    \item Established Connection: (IP, Port, L4 (Ack to Write)). We choose an acknowledgement to a client's write as being a measure for establishing a connection because...\todo{fill in}.
    \item S/A: (IP, Port) We find many IP in the wild which acknowledge a syn scan yet can never actually establish a connection (e.g., S/A comes with a window size of 0, the IP RSTs after our client completes the handshake). 
\end{itemize}






\subsection{Classifying Ports based on Popularity}

\subsubsection{Syn/Ack Popularity}

Throughout our analysis we refer to certain ports as being S/A-Super-Common, S/A-Common, and S/A-Uncommon, based on the number of Syn Acks received when scanning a particular port. We determine which ports fall into which category by conducting three differently-seeded concecutive 0.1\% scans of IPv4 on all 2\^32 ports --- each scan taking ~ 2.5 days --- and take the average number of S/As returned on each port across the three scans. We validate that our 0.1\% sample is sufficient to compare S/A popularity of ports relative to each-other by conducting 100\% scans of the reported top 20 ports and 2 other random ports and validating that 1. the number of S/As collected in the 0.1\% scan is 0.1\% of the S/As collected in the 100\% scan (within an error of 0.001\%), 2. The relative rankings of the top 20 ports in the 0.1\% scans stays consistent when scanning at 100\%.  We plot the S/A-popularity of ports in Figure~/\ref{fig:sa_popularity}. We apply Grubb's test \todo{cite}, a non-parametric statistical outliers test, with a 99.99\% confidence iteratively to find clusters of port S/A popularity. Grubb's test finds 3 clusters of S/A popularity: 6 Super-Common ports, 90 Common Ports, and 65439 Uncommon ports. 

\begin{figure}[H]
  \centerline{\includegraphics[width=\linewidth]{figures_paper/port_popularity.pdf}}
  \caption{ S/A Port Popularity -- \textnormal{ Three clusters, based on S/A popularity, of ports exist. }}
  \label{fig:sa_popularity}
\end{figure}

The six ports which receive the most number of Syn/Acks are port 80 (HTTP),443 (HTTPS),7547(CWMP),22(SSH),30005 (Router Remote Management), and 5060 (SIP). Note that port 30005 is not widely accepted as a common port, most likely due to its high number.  

\subsubsection{Network Popularity}

We scan the top 30 most common ports at 100\% and are surprised to find that the number of unique Autonomous Systems responding on each port is not correlated with the number of Syn/Acks received; Port 80 (58196 unique networks), Port 443 (59316 unique networks), Port 7547 (10793 unique networks), Port 22 (46551 networks), and port 30005 (10113 networks). We attempt to cluster all ports scanned at 1\% based on network diversity, but find that scanning at 1\% is not sufficient to detect network diversity as scanning a subsample of IPv4 is biased towards sampling more dense Autonomous Systems. In Figure~\ref{fig:net_popularity} we depict using different sizes of subsamples of IPv4 to rank ports based on network popularity causes incorrect and inconsistent ranking. For example, sub-sampling at 1\% will cause over half of the ports to be ranked incorrectly. Ports which are more likely to appear in sparse networks are more greatly affected by subsampling. 

\begin{figure}[H]
  \centerline{\includegraphics[width=\linewidth]{figures_paper/as_rank_net_diversity.pdf}}
  \caption{ Network-Diversity Port Popularity -- \textnormal{ Ports 80,443,22,53 and 21 appear in the most number of unique autonomous systems. Note that when subsampling IPv4, the # of unique autonomous systems scanned is not consistently relative to other ports and can therefore produce incorrect network-diversity rankings.  }}
  \label{fig:net_popularity}
\end{figure}





\subsubsection{1\% vs 100\% and the biases of scanning}

> 




==> redacted.tex <==

%85\% likelihood of responding with a \sa on port 179; intuitively this is rather
%unexpected and strange since there are no known correlations between the Modbus
%and BGP services. It turns out the high correlation of response between the two
%unlikely ports \textemdash and most of the behaviors that lead to a \sa{ing}
%server not accepting data \textemdash is due to firewalls which operate on large
%sub-nets of IPs. Moreover, these firewalls  \sa on nearly all ports, which is
%evidenced by the relatively constant \textit{raw number} of IPs which \sa yet
%can only reach the established or receives data state (Figure~\ref{fig:l4_all}).
%
%In the following two subsections we will traverse the TCP state diagram (Figure~\ref{fig:flowchart}) and describe in detail why hosts (1) never make it past the established state, and   (2) never make it past the receives data state. We will also show which types of firewalls and middleboxes behave in corresponding to the strange TCP behavior and where and at which network granularity these firewalls are implemented.

%In fact, we discover that ports which are known to be
%associated with critical vulnerabilities (``security sensitive ports'' such as
%BGP \cite{CVE-2011-2760})  are the most likely to send a \sa yet not accept
%data. Another example is port 502 (Modbus), a port that has numerous common
%vulnerabilites and exposures (CVEs)
%\cite{CVE-2007-4827,CVE-2008-7199,CVE-2011-4861,CVE-2013-2784,CVE-2013-5741,CVE-2017-7575,CVE-2018-5400,CVE-2019-9590},
%in which 80\% of servers which \sa do not accept data.

%our results for the original 44 IANA-assigned ports and an extra selection of the 17 most popular random ports. The L4 breakdown of TCP state (established, receives data, accepts data) of the remaining random ports is nearly identical to the less-popular (i.e., random ephemeral ports) ports in Figure~\ref{fig:l4_all}.


%We next test whether all IP/Port pairs which \sa can actually accept data by using our custom module on a random 1\% of the public IPv4 address space on a random subset of 2,000 ports and the original 44 IANA assigned ports. We verify our results are consistent with 3 differently seeded 1\% scans. We also verify that our 1\% scans provide an accurate breakdown of IP/Port behavior compared to a 100\% scan, by also using our custom ZGrab module on 11 IANA assigned ports and 13 random ports on 100\% of the IPv4 address space. We run the different seeded 1\% scans in September and October of 2019 (each taking a week) and run the 100\% scans in October 2019 (taking 2 days to complete). All scans are run from one server scanning at 50k packets per second (to minimize packet drop).


%Figure~\ref{fig:l4_all} illustrates the breakdown of the three states \textemdash corresponding to the highlighted states TCP Flow chart \rt{It is very hard to see this in my black and white version. Maybe better to keep states in black and just discuss?} in  \textemdash for which a responding IP (i.e., one that sends a \sa on our custom ZGrab module), can reach. The grey is the fraction of all IPs which only reach the established state but cannot receive data (i.e., \sa with a window size of 0). The orange is all IPs which can reach both the established and receives data state but for some reason (e.g., abruptly closes the connection, never responds with an \ack ) will not accept data. The blue is all IPs which successfully \ack the 1 byte of data that is sent by the custom module.


%On ephemeral ports \todo{which},ASes that respond contain at least one
%IP which \sa with a window size of zero that never acknowledges data. On a common
%port like 80, however, only 3\% of responding ASes \sa with a zero window.
%\todo{Is this of \emph{all} ASes? This does not make sense. Why would it be an
%order of magnitude different if we think they respond on all ports? If it's
%not.... what are the ports with the most zero window IPs or networks? This isn't
%really explained anywhere and it's much too small in the upper part of Fig 3 to
%understand} \rt{I added ASes that respond to make this clearer, but I do think
%that maybe adding the absolute numbers would help. I assume the raw number of
%ASes that respond will be similar for the different ports.} \todo{+1}

%\begin{figure}[h]
%  \centerline{\includegraphics[width=\linewidth]{figures_paper/syn-sent-asn_v_ip_fracs.pdf}}

%%  \caption{ \textbf{Distribution of \syn-sent firewall behaviors across ASes} ---%
%  \todo{change to bar graph and only perc ASes?}
%  On a common port like 80, \syn-sent firewall behaviors are each present in less than 20\% of responding ASes. On an uncommon port like the random ephemeral port 49227, ZeroWindow \sa is present in near 30\% of responding ASes. Dynamic blacklisting after a handshake is only 5\% of responding ASes yet affects over 30\% responding IPs because the ASes that  dynamically blacklist do so on a lot of IPs.  }
%  \label{fig:db_asnipfracs}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[h]
%  \centerline{\includegraphics[width=1.2\linewidth]{figures_paper/syn-sent_handshakes.pdf}}
%  \caption{\textbf{ A \sa is not equivalent a TCP established state}---%
%  IPs which fail to reach the TCP established state do so for 3 primary reasons. The breakdown of the behaviors stays fairly constant across ports because IPs which exhibit these behaviors are very likely to do so across all ports. Notable exceptions are security-relevant ports 445 (SMB) and 502 (Modbus) due to Network-Wide blocking, discussed in Section~\ref{sub:sec:security_impl}.}
%  \label{fig:l4_no_syn}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%40\% of IPs seem to
%do it solo. Upon further investigation, we notice that those IPs are often
%surrounded by other IPs which reset the connection (12\% of IPs reset the
%connection in solo, as seen in Figure~\ref{fig:es_cdf}). We investigate whether
%the difference in behavior is somehow correlated with the likelihood of an IP
%running a real service on another port but do not find a clear relationship.

%We discover that if a server dynamically blacklists on one port and the client
%continues to use the same source-IP to probe, every port which fails to
%acknowledge data becomes dynamically blacklisted (i.e., scanning a new ephemeral
%port will no longer \sa). We confirm with a new experiment using different
%source-IPs that using a new source IP evades dynamic blacklisting due to
%\syn-scanning  and will again prompt the host to \sa.

%all packets are dropped
%
%from the
%ZMap IP address (85\% of IPs drop subsequent packets across ports); (2) the host
%explicitly resets the connection (10\% across ports); and (3) the connection is
%ICMP prohibited (5\% across ports).
%
%after an attempted connection\rt{are the following
%percentages over the hosts that only respond in the first scan?}:

%We investigate dynamic blacklisting with back-to-back scans to test how many IPs
%will consistently respond across all scans. Using ZMap, we perform five
%single-packet TCP \syn scans of 1\% of the public IPv4 address space using the
%same seed and same source IP on the same 61 ports from the experiment set-up in
%Section~\ref{sub:sec:tcp_state}. We space the starting time of each scan to be
%one-second apart from each other. We then compare the results of the first scan
%with the latter scans. In November~2019, we conduct this experiment four times
%using a different source IP address each time and verify that the results are
%consistent.

%Between 1--8\% of all responding IPs, depending upon the port, will only \sa on
%the first scan.  Moreover, 7\% of ASes experience at least one failed follow-up
%handshake across all scanned ports and half of such ASes experience between a
%3\%--100\% subsequent-handshake failure rate.



%First, we verify that \lmap's fingerprinting (discussed in
%Section~\ref{sub:sec:fingerprinting}) correctly identifies expected services.
%Fingerprinting allows \lmap to identify services without having to complete an
%entire L7 handshake (e.g., using ZGrab). We find that \lmap is able to identify
%all of ZGrab's expected services with just the first packet.\todo{this needs to
%be explicit that it's the first packet of each service. Also, why would this be
%surprising?} Moreover, \lmap can identify more HTTP services (e.g., port~80 and
%port~62220 in Table~\ref{table:comp_zgrabs}) due to certain HTTP re-directs
%only responding to the first L7~handshake (i.e., \lmap). \todo{What? Why/How
%are they different? If it's simply the first L7 handshake, ZGrab would also
%find them.  Explain what's going on.}
%and 90~IPs using six additional protocols on port 27017 (SMTP, SSH, RFJS, FTP,
%RocketRcon, VNC).

%The breakdown of the unexpected services is, unsurprisingly, nearly identical
%to the distribution in Figure~\ref{fig:hist_services}.
%
%The number of filtered IPs with \lmap is consistently lower than the number
%filtered with ZMap as we can see in Table~\ref{table:comp_zgrabs}. As a result
%the L7 scan with ZGrab is considerably faster---the total runtime speed up is
%at least 1.3x (for port 443). Note that the speed-up is not at all surprising;
%for example, the number of IPs which actually acknowledge data on port 27017 is
%an order of magnitude less, consistent with results from
%Section~\ref{sub:sec:tcp_state}.
%
%The speedup on the L7 scanning phase comes at the cost of a more elaborate
%filtering phase (using Algorithm~\ref{fig:alg_2}). We estimate the performance
%overhead of \lmap to be negligible.  Due to the pipelined and stateless nature
%of ZMap+\lmap, we expect that the collection of \ack{s} will be contained
%within the original ZMap runtime + default cool-down period and thus not
%encounter any runtime overhead.
%\rt{Maybe we can remove this paragraph.}
%We further investigate the effect of the selected data on host acknowledgement with
%our experiment setup from Section~\ref{sec:l4}, but varying the data sent. We verify
%whether there are IPs that successfully complete the expected L7 handshake but do not
%acknowledge non-compliant RFC data (e.g., two newline characters). Across 73\% of ports
%scanned, less than 0.1\% of IPs do not acknowledge the two newline characters. IPs on Port 22
%that SSH are the most selective to acknowledge; up to 0.9\% of IPs will not acknowledge
%two-newlines but do acknowledge data containing the plaintext ``SSH.'' Middleboxes such as
%SmartXFilter will \rst the connection if the sent data does not meet the expected standards. On
%port 80, hosts running SmartXFilter make up 22\% of the IPs that filter. These hosts will
%\textit{only} respond to an RFC-compliant GET Request.





==> scraps.tex <==


\subsubsection{S/As and Port Popularity are not always correlated}
\label{subsub:sa_not_cor}

% trim={<left> <lower> <right> <upper>}




It could be argued that though S/As do not precisely measure the number of real services running on an IP/port, if S/As are still an appropriate measure to approximate the relative popularity

For a network such as AWS (ASN\,16509) network (Figure~\ref{fig:l4_aws}, for example, the fraction of established connections is undeniably still highly correlated with the relative port popularity. Thus, relatively speaking, using S/As as a proxy to, for example, measure relative port popularity, is still fine.



\begin{figure}[H]
  \centerline{\includegraphics[width=\linewidth]{figures_paper/handshakes_AWS.pdf}}
  \caption{ Amazon Web Services L4 Dynamics -- \textnormal{As port s/a popularity decreases, so does the likelihood of an IP keeping an open TCP Connection. }}
  \label{fig:l4_aws}
\end{figure}


However, correlation between S/As and the fraction of IPs which can actually keep a TCP Connection open is not present in all networks; measuring the top 5 most popular ports using S/As produces an incorrect "top 5 ports list" for 27\% of scanned networks. Within just the top 10 largest scanned networks (based on overall S/As), 50\% of the networks  produces an incorrect "top 5 ports list."

For example, Based on overall number of S/As received across all ports, Korea Telecom (ASN\,4766) is labeled as the largest scanned network. However, due to the majority of S/As on port 7547 being followed by F/As, it is not possible for us to scan the CWMP service and thus, from our scanner's perspective, is incorrectly labeled as the most popular port. Misleading responses on 7547 also incorrectly imply that Korea Telecom is the largest scanned network.

\begin{figure}[H]
  \centerline{\includegraphics[width=\linewidth]{figures_paper/handshakes_koreaTelecom.pdf}}
  \caption{ No Correlation between S/As and Open TCP Connections   -- \textnormal{Due to the majority of S/As on port 7547 being followed by RSTs, port 7547 does not host a public CWMP service and is thus incorrectly labeled as the most popular port. Misleading responses on 7547 also incorrectly imply that Korea Telecom is the largest scanned network. }}
  \label{fig:l4_korea}
\end{figure}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{AWS vs. ISP example of weirdness?}
\todo{discuss how some networks do not have  a lot of the strange behavior discussed and therefore L4 estimation }





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Limitations of Module}
\label{subsub:limitations}

Misses x\% of redirects.... though we scan for http redirects explicitly in the latter sections so we account for that.
also one could argue that since the page is redirecting, it technically isnt hosting a service itself.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{TTL values: evidence of a firewall}

Prior work has used mismatching TTL values to detect the presence of firewalls and middleboxes \todo{cite}. Across ports, the same IP might exhibit different TTL values due to load balancing, for example. \todo{cite}. Mismatching TTLs could also show up if an alternate route was taken to/from the IP. Middleboxes can also artificially change the TTL value so that they always appear the same. Thus, it is undeniably hard to read into mismatching TTLs. 

Across all ports scanned, 16.8\% of IPs have mismatching TTLs on the same port scanned and 38\% of IPs have mismatching TTLs across all ports scanned. 


However, we further find a behavior present almost exclusively in these blacklisting networks where on ports which do not accept data, the TTLs values are the same across TCP responses whereas the TTL values are different across TCP responses on the same port. 

As a result, 

We discover that the increase is due to whether the IP contains at least one port which can accept data. In other words, A \sa on a port that exhibits no evidence of establishing a TCP connection will hold a different TTL value than a \sa on a port which can eventually establish a TCP connection.

Thus, when filtering for IPs which can accept data on at least one port, 66\% of scanned IPs have mis-matching TTLs. 45\% of such IPs have mismatching TTL on the same port, whereas thee rest have mis-matched TTLs \textit{across} ports. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Analyzing Intrusion Detection Systems at the network granularity}

\todo{discuss looking into internals of nets. num of ports per category ? TTL values? merge canada thing here? or port blocking here?}


We, find IDS L4 behavior wide-spread across networks; 43\% of all scanned network contain at least one IP/Port pair which send a \sa but cannot accept data. The wide-spread nature is perhaps unsurprising since the usage of firewall/ IDS usage is now commonplace \todo{cite}. However, we also find a small subset of networks are more likely to have an L4 discrepancy; 0.6\% of all networks scanned make up 80\% of the \sa which will never accept data. 

This is due to the fact that in some networks, over 99\% of responses received on a port will be consistent with IDS behavior and thus not be hosting a real service. Across all networks scanned during select 100\% scan of non-common ports (e.g., 8883,1911,2000) roughly 50\% of networks which contain at least one IDS-like \sa,  \textit{only} (i.e., greater than 99\% of IPs) respond with IDS-like \sa. We also notice that for some large common networks, such as Chinanet (AS\,4134), the firewall-like behavior is not present throughout the entire network, yet is present in clusters of IPs throughout the network. For example, in 11\% of networks with at least one IP that sends a \sa yet does not accept data, the overall fraction of IP,Port pairs which do not accept data is less that 99\%,  yet the likelihood that the immediate neighbor of an IP exhibits identical behavior is greater than 50\%. For 5\% of networks, the likelihood is greater than 80\%.

In general, we find that larger networks are more likely to exhibit more than one type of \sa category.  Out of the top 100 largest scanned networks, 95\% exhibit more than one type of \sa. Across all scanned networks,

Within some ASes, the non-authentic \sa are present \textit{mostly} network-wide; 26\% of these ``0.6\% top misbehaving'' ASes will respond with a non-authentic \sa across 99\% of (IP,Port) pairs which return a \sa. 74\% of these Ases will respond with a non-authentic \sa across over 50\% of (IP,Port) pairs which return a \sa. 


21\% of scanned networks  exhibit more than one type of \sa.  We suspect that networks which exhibit multiple \sa categories of behavior are due to spacial locality (i.e., IPs exhibiting the same behavior will be grouped together). To further investigate this hypothesis, we conduct a 100\% scan of UK Regional Network (AS\,2856) --- a network which exhibits the largest number of firewall behaviors across all 5 \sa categories--- on a select 7 ports and through manual inspection of IP address space find evidence spatial locality. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We discover two compelling reasons \textemdash one a the host granularity and one at the network granularity \textemdash for a TCP connection to be immediately closed after a handshake. 

First, if an individual server does not want to communicate with the client (e.g., due to mismatches in ``security clearances,'') RFC 793 advises that the server should close the TCP connection after the client acknowledges the \sa. Consequently, an individual host might still \sa before closing the connection. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\todo{ports which look ephemeral but are actually commonly assigned to services (30005)}

\subsubsection{Scanning Implications from Dynamic Blacklisting}


Dynamic Blacklisting has direct implications to scanning because it is common for prior work to use two-phased scanning. By attempting to perform a follow-up application layer scan on an IP which has now dynamically blacklisted the scanner, the scanner thus suffers in performance as it is keeping an open connection dedicated to an IP/Port pair which will never actually respond.

Dynamic blacklisting behavior also (1) Causes a discrepancy between the first time a \syn-Scan is run compared to subsequent times. (2) Biases results depending upon whether multiple source IP addresses are used.

We discover that 6\% of IPs blacklist so quickly that, when we repeat our dynamic-blacklisting \syn-scan experiment except send multiple probes from the same source IP, the IPs will consistently only respond to the first probe. Therefore, a stateless \syn-scanner can conveniently choose to immediately filter such IPs out by considering the number of responses received (e.g., only one \sa out of an expected three).

Dynamic blacklisting can also potentially conflate analysis of packet loss due to a poor TCP connection if only looking at L4. Prior work attributes a probability of around 2\% packet loss when syn-scanning with one probe \cite{durumeric2013zmap}. We discover however that certain networks exhibit a much larger than 2\% packet loss; 7\% of ASes experience at least one failed follow-up handshake across all scanned ports and 50\% of such ASes experience between a 3\% - 100\% subsequent-handshake failure rate.



\todo{need to figure this section out...}


\subsubsection{Firewalls which drop all traffic}
\label{sub:sub:sec:drop_all}

%We also notice that it is common for networks to drop all traffic (both \sa and \rst) destined towards security sensitive ports. Out of the top 50 ASes which \sa the most in our scan, we find 28\% of these top 50 networks drop all packets pertaining to port 445 (SMB), 10\% drop port 23 (Telnet) and 10\% drop port 11211 (Memchached). Akamai, drops all traffic not pertaining to ports 443 (HTTPS) and 80 (HTTP).

Traffic filtering by dropping at the network level actually decreases the likelihood of an IP/port responding with a large number of \sa which do not accept data.  For example, port 445 (SMB) is known to be highly security sensitive due to incidents such as WannaCry \cite{wannacry} and is thus the most commonly blocked port. The networks that block port 445 also happen to be the networks with the largest number of IPs which do not accept data across all ports scanned. Consequently, port 445 is 50\% more likely to host legitimate services than its neighboring ports in popularity, as depicted in Figure~\ref{fig:l4_all}.

\todo{leftover}
DDos protection is actually pretty common...especially in bigger networks. Information leakage from firewalls.

We also notice that it is common for networks to drop all traffic (both \sa and \rst) destined towards security sensitive ports. We discover that the  top 5 ports which experience the largest fraction of firewall behaviors that still send a \sa are all security-relevant ports:
ports 502 (Modbus) ,102 (s7) \cite{102CVE-2016-3949,102CVE-2016-2201,102CVE-2016-2200,102CVE-2015-8214,102CVE-2015-2822,102CVE-2015-2177,102CVE-2015-1601,102CVE-2013-0700} ,11211 (Memchached) \cite{11211CVE-2018-1000115,11211CVE-2011-4971},27017 (Mongodb) \cite{27017CVE-2015-1937]} and 179 (BGP). 


\textbf{Honeypots} Fingerprinting services on ports leads to discovering honeypots and infected devices~\cite{bitterharvest,detectmeifyou,mirai}. 

Fingerprinting techniques have primarily focused on scanning for protocols on expected ports. We classify hosts which successfully respond with multiple unexpected service on the same port and find an estimated 33,000 hosts in AWS (ASN\,16509, 14618) which run http, mqtt, redis, tls, and ssh on 20 non-ephemeral ports (e.g., 993, 8443). \todo{describe}

With the advent of honeypots, such as T-Pot~\cite{tpot}, are likely to be running more than one honeypot \todo{botnet example?}, we encourage future work to consider fingerprinting for multiple services on the same port.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[h]
\centering
\small
%\smallca
\begin{tabular}{llll}
\toprule
%\# IPs & \#L7 & speed-up \\
Port &
\multicolumn{3}{c}{Output: Expected Services $\pm$ std.\ dev.} \\ \cmidrule(r){2-4}
	& SYN-ACK  & ACKs \texttt{\textbackslash{n}\textbackslash{n}} & ACKs L7   \\
\midrule
80/HTTP    & 543K $\pm$ 976 & 541K $\pm$ 1083 & 542K  $\pm$ 1426  \\
443/TLS    & 465K $\pm$ 665 & 461K $\pm$ 689  & 465K $\pm$ 787   \\
22/SSH     & 172K $\pm$ 709 & 165K $\pm$ 532  & 167K  $\pm$ 4503   \\
27017/Mongo& 924 $\pm$ 1 & 924 $\pm$ 1&  924 $\pm$ 1\\
\bottomrule
%100\% & Port 80 (HTTP) & 65,702,046 &  3h28m & 53,516,645 & 61,206,625 & 2h53m & 53,450,208  \\
%44,558,220 + 8958425 app-err for all and 44,523,367 + 8926841 for ack

%100\% & Port 502 (Modbus) & & \TK  & & & \TK  \\
%\bottomrule
\end{tabular}
	\caption{\textbf{\lmap Impact on Scan Results}---%
	LZR significantly increases L7 scan performance on ports without many
	expected services by sending data in an \ack packet and checking the
	server's response. Sending the first packet of the expected L7 handshake
	does not have statistically significant result on results. Sending two
	newline characters is generic across all ports, but incorrectly filters out
	a small percentage of hosts that would have otherwise completed a normal L7
	handshake.
	}
\label{table:comp_output}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
